Variational Bayesian Pseudo-Coreset

The success of deep learning requires large datasets and extensive training, which can create significant computational challenges. To address these challenges, pseudo-coresets, small learnable datasets that mimic the entire data, have been proposed. Bayesian Neural Networks, which offer predictive uncertainty and probabilistic interpretation for deep neural networks, also face issues with large-scale datasets due to their high-dimensional parameter space. Prior works on Bayesian Pseudo-Coresets (BPC) attempt to reduce the computational load for computing weight posterior distribution by a small number of pseudo-coresets but suffer from memory inefficiency during BPC training and sub-optimal results. To overcome these limitations, we propose Variational Bayesian Pseudo-Coreset (VBPC), a novel approach that utilizes variational inference to efficiently approximate the posterior distribution, reducing memory usage and computational costs while improving performance across benchmark datasets.

==> main/problem_setup.tex <==
\section{Problem setup}
\label{sec:problem_setup}
({\color{red} This section will be removed and merged into 4.1})    
Consider a supervised learning problem with an empirical dataset distribution $\calD:=\frac{1}{n}\sum_{i=1}^n\delta_{(x_i,y_i)}$ where $\delta$ denotes the Dirac measure. Given a model $f_\theta$ with parameter $\theta$, we solve the variational optimization problem to obtain an approximate posterior with natural parameter $\lambda$ as follows:
\begin{align}
\lambda_{\calD}^*=\argmin_{\lambda}\calL_\calD(\lambda):=\argmin_{\lambda}\bbE_{(x,y)\sim \calD}\bbE_{q_\lambda}\left[-\log p_\calD(y|x,\theta)\right] + \KL\left[q_\lambda||p_{\lambda_0}\right],    
\end{align}
where variational posterior distribution $q_\lambda$ and weight prior distribution $p_{\lambda_0}$ are defined by
\begin{align}
    q_\lambda(\theta)\propto \exp\left(\left<\psi(\theta), \lambda\right>-A(\lambda)\right),\;&\;p_{\lambda_0}\propto \exp \left(\left<\psi(\theta), \lambda_0\right>-A(\lambda_0)\right),
\end{align}
and $p_{\calD}(y|x,\theta)$ is the pre-defined likelihood distribution. Then our goal is to learn a synthetic dataset distribution $\calS$ where the optimal variational posterior natural parameter $\lambda_{\calS}^*$, which is obtained from variational optimization problem utilizing $\calS$, well approximates $\lambda_{\calD}^*$. Our goal here is to ensure that the number of parameters needed to define $\calS$ is significantly smaller than the number of parameters required to represent the dataset distribution $\calD$. By doing so, we aim to reduce the memory required to store the data and the training cost needed for learning, while still achieving a good variational posterior. The variational optimization problem utilizing $\calS$ is formulated as follows:
\begin{align}
    \lambda_{\calS}^* = \argmin_\lambda \calL_{\calS}(\lambda):=\argmin_\lambda\bbE_{(x,y)\sim\calS}\bbE_{q_\lambda}\left[-\log p_\calS(y|x,\theta)\right] + \KL\left[q_\lambda||p_{\lambda_0}\right],
\end{align}
where $p_{\calS}(y|x,\theta)$ is the likelihood distribution for the synthetic dataset distribution. To learn optimal $\calS$, we solve the following bilevel optimization problem:
\begin{align}
    \calS^* = \argmin_S \calL_\calD(\lambda_\calS^*)\quad
    \text{where}\;\; \lambda_\calS^* = \argmin_\lambda \calL_\calS(\lambda).
\label{eq:bilevel}
\end{align}
